Immersed boundary simulations of cell-cell interactions in whole blood

We present a new method for the geometric reconstruction of elastic surfaces simulated by the immersed boundary method with the goal of simulating the motion and interactions of cells in whole blood. Our method uses parameter-free radial basis functions for high-order meshless parametric reconstruction of point clouds and the elastic force computations required by the immersed boundary method. This numerical framework allows us to consider the effect of endothelial geometry and red blood cell motion on the motion of platelets. We find red blood cells to be crucial for understanding the motion of platelets, to the point that the geometry of the vessel wall has a negligible effect in the presence of RBCs. We describe certain interactions that force the platelets to remain near the endothelium for extended periods, including a novel platelet motion that can be seen only in 3-dimensional simulations that we term "unicycling." We also observe red blood cell-mediated interactions between platelets and the endothelium for which the platelet has reduced speed. We suggest that these behaviors serve as mechanisms that allow platelets to better maintain vascular integrity.

==> cell-models.tex <==
\section{Cell models}\label{sec:models}
This section is composed of two subsections. The first is dedicated to RBCs and
platelets, which while very different biologically, are quite similar for modeling
purposes. The second subsection deals with the endothelium.

\subsection{Red blood cells and platelets}

The membranes of RBCs and platelets are topological spheres, so we use the spherical
parametrization
\begin{equation}
    \Xp_{\sphere}(\qs) = \left[\begin{array}{c}
            \cos\q[1]\cos\q[2] \\
            \sin\q[1]\cos\q[2] \\
            \sin\q[2]
    \end{array}\right],
\end{equation}
for $\qs\in(-\pi,\,\pi]\times[-\pi/2,\,\pi/2]$, to parametrize both kinds of membranes.
For any two points on $\sphere$,
$\Xp_A = \Xp(\qs_A)$ and $\Xp_B = \Xp(\qs_B)$, the distance between them is given by
\begin{equation}
    \begin{aligned}
        \left\|\Xp_A - \Xp_B\right\|
        &= \sqrt{2\left(1-\Xp_A\cdot\Xp_B\right)} \\
        &= \sqrt{2\left(1-\cos\q[2]_A\cos\q[2]_B\cos\left(\q[1]_A-\q[1]_B\right)+\sin\q[2]_A\sin\q[2]_B\right)}.
    \end{aligned}
\end{equation}
That the distance is a function only of the angle between two points implies that the
sphere is homogeneous~\cite{Fuselier:2013coba}, and therefore suitable for computing
quadrature weights. Its surface area is $\area{\sphere} = 4\pi$. This
parametrization has Jacobian $\tilde{J} = \cos(\q[2])$, which vanishes at the
poles, $\q[2] = \pm\pi/2$. The quadrature weights~\eqref{eq:quad-cov} require that the
Jacobian not vanish. We choose data and sample sites away from the poles to avoid any
issues. For this, we use the Bauer spiral~\cite{Bauer:2000km},
\begin{equation}
    \begin{aligned}
        \q[2]_A &= \sin^{-1}(-1 + (2A-1) / N) \\
        \q[1]_A &= \sqrt{N\pi}\q[2]_A - 2\ell\pi,
    \end{aligned}
\end{equation}
where $N$ is the number of sites, $\data\cardinality$ or $\sample\cardinality$, and
$\ell$ is an integer chosen so that $\q[1]_A$ falls in the range $(-\pi,\,\pi]$.

RBCs have viscoelastic membranes. The Skalak Law was developed specifically for the RBC
membrane~\cite{Skalak:1973tp}. We use  The reference shape of the RBC is given by~\cite{Omori:2012hw}
\begin{equation}\label{eq:rbc-shape}
    \reference\X_\text{RBC} = 3.91\um\left[\begin{array}{c}
            \cos\q[1]\cos\q[2] \\
            \sin\q[1]\cos\q[2] \\
            p(\cos\q[2])\sin\q[2]
    \end{array}\right],
\end{equation}
where $p(r) = 0.105 - r^2 + 0.56r^4$.


\subsection{Endothelium}
The endothelial layer is a patchwork of endothelial cells lining the blood vessel. We 
treat these cells as a single object that covers the entirety of the bottom of the
domain. Endothelial cells are held fast to the subendothelium. We therefore consider
the endothelium to consist of damped springs with spring constant $k=$ % XXX
and damping constant $\eta=$. % XXX
Because these forces do not require any data outside of position and surface velocity,
we do not need to invoke the RBF machinery described in section~\ref{sec:surfaces}.
Instead, the endothelium is represented by a collection of points. 

Parametrization:
\begin{align*}
    \q^2_A &= 2\pi (A-1)/N,
    \q^1_A &= \left\lceil\!\sqrt{N}\mskip\thinmuskip\right\rceil\theta^2_A - 2\pi\ell,
\end{align*}
where $N$ is the number of points, $A$ ranges between 1 and $N$, and $\ell$ is chosen so
$\q^1_A$ falls in the range $(0,\,2\pi]$.

%Because of the periodicity of the domain, the endothelium is topologically a
%torus. To parametrize a torus, we use the parametrization
%\begin{equation}
%    \Xp(\qs) = \left[\begin{array}{c}
%            \cos\q[1] \\
%            \sin\q[1] \\
%            \cos\q[2] \\
%            \sin\q[2]
%    \end{array}\right],
%\end{equation}
%for $\qs\in[0,\,2\pi)^2$, which is used only for defining the parametric distance,
%\begin{equation}
%    \begin{aligned}
%        \left\|\Xp_A - \Xp_B\right\| 
%        &= \sqrt{2 - \Xp_A\cdot\Xp_B} \\
%        &= \sqrt{2-\cos(\q[1]_A-\q[1]_B)-\cos(\q[2]_A-\q[2]_B)},
%    \end{aligned}
%\end{equation}
%and therefore finding that $\mathbb{T}$ is homogeneous with surface area
%$\area{\mathbb{T}} = 4\pi^2$.
%
%{\color{red}Forces here?} % TODO

We are interested in investigating two flow regimes in particular, characterized by the
shear rate, $\shear$. When exposed to a low shear rate, the endothelial cells arrange
themselves in a cobblestone pattern, while a high shear rate will elongate the
endothelial cells in the flow direction~\cite{Nerem:1985ty,Levesque:1986tc}.


==> rbf-interpolation_new.tex <==
\subsection{Surface reconstruction with radial basis functions}

In this section, we discuss the problem of modeling and reconstructing surfaces diffeomorphic to the 2-sphere $\sphere$ from point-clouds using RBFs. Consider the 2-sphere, $\sphere$, with parametrization
\begin{equation*}
    \Xp(\qs) = \cos\q[1]\cos\q[2]\e_1 + \sin\q[1]\cos\q[2]\e_2 + \sin\q[2]\e_3,
\end{equation*}
$\qs\in\sites = (-\pi,\,\pi]\times[-\pi/2,\,\pi/2]$. Let $\data\sites = \{\qs_i\}$ be a
set of $\data\cardinality$ distinct \emph{data sites}, and $\data\Xp_i = \Xp(\qs_i)$ for
each $\qs_i \in \data\sites$. We use the Bauer spiral~\cite{Bauer:2000km} to generate a
quasi-uniform set of $N$ points on the sphere in parallel:
\begin{equation}
    \begin{aligned}
        \q[2]_i &= \sin^{-1}(-1 + (2 i - 1) / N), \\
        \q[1]_i &= \pi - \modulo\left(\pi - \sqrt{\pi N} \q[2]_i,\,2\pi\right).
    \end{aligned}
    \label{eq:bauer-spiral}
\end{equation}
We now describe the process of approximating a general function $\psi(\Xp) : \mathbb{S}^2 \to \mathbb{R}$ using RBF interpolation. The RBF interpolant can be written as:
\begin{equation}
    s(\data\Xp)
    := \sum_{i=1}^{\data\cardinality} c_i \phi\left(\left\|\data\Xp-\data\Xp_i\right\|\right)
    + \sum_{k=1}^{\poly\cardinality} d_k p_k(\data\Xp),
    \label{eq:interpolant}
\end{equation}
where $\phi(r)$ is a radial basis function and $\{p_k(\Xp)\}$ are the $\poly\cardinality$ spherical harmonics on $\mathbb{S}^2$. Regardless of the choice of $\phi$, we may find a unique set of interpolation coefficients $c_i$ and $d_k$ by imposing the following pair of conditions on the interpolant:
\begin{align}
s\left(\data\Xp_j\right) &= \psi(\data\Xp_j), j=1,\ldots,\data\cardinality, \label{eq:interp_constraints} \\
\sum_{i=1}^{\data\cardinality} c_i p_k(\data\Xp_i) &= 0. \label{eq:constraints}
\end{align}
The constraint~\eqref{eq:interp_constraints} imposes that the interpolant exactly matches samples of $\psi(\Xp)$ at the given $\data\cardinality$ points, while the constraint~\eqref{eq:constraints} forces the interpolant~\eqref{eq:interpolant} to reproduce spherical harmonics up to a specified degree~\cite{Fuselier:2013coba,SWJCP2018}. In this work, we select $\phi$ as the polyharmonic spline (PHS), defined as
\begin{equation*}
    \text{PHS:}\quad\phi(r) = \begin{cases}
        r^k \log r, & \text{for even exponents } k \ge 2 \\
        r^k, & \text{for odd exponents } k \ge 1,
    \end{cases}
\end{equation*}
which do not require a shape parameter, unlike Gaussian or multiquadric kernels~%
\cite{Fasshauer:2007ui}. The constraints~\eqref{eq:interp_constraints} and~\eqref{eq:constraints} can be collected into a block system:
\begin{align}
\underbrace{\begin{bmatrix}
A & P \\
P^T & 0
\end{bmatrix}}_{\tilde{A}}
\underbrace{\begin{bmatrix}
\underline{c} \\
\underline{d}
\end{bmatrix}}_{\tilde{\underline{c}}} =
\underbrace{\begin{bmatrix}
\underline{\psi} \\
0
\end{bmatrix}}_{\tilde{\underline{\psi}}}, \label{eq:rbf_linsys}
\end{align}
where
\begin{align}
A_{ij} &= \phi\left(\left\|\data\Xp_i-\data\Xp_j\right\|\right), i,j=1,\ldots\data\cardinality,\\
P_{ij} &= p_j(\data\Xp_i), i=1,\ldots,\data\cardinality, j=1,\ldots,\poly\cardinality,\\
\vec{\psi}_i &= \psi(\data\Xp_i),i=1,\ldots,\data\cardinality.
\end{align}
The matrix A arising from the PHS kernels is conditionally positive definite, but the additional polynomial terms are sufficient to guarantee a unique solution to the above linear system~\cite{Fasshauer:2007ui,Wendland2004}.

This technique can be extended in a straightforward fashion to vector-valued functions by using a separate set of coefficients for each component of the vector, and turning the right hand side of~\eqref{eq:rbf_linsys} into an $\data\cardinality \times d$ matrix, where $d$ is the number of vector components~\cite{Shankar:2015km}.  More precisely, suppose that $\X(\qs)$ is a parametrization of $\interface$, e.g., the membrane of an RBC. We identify the point $\X(\qs)$ on $\interface$ with the point $\Xp(\qs)$ on $\sphere$. Each component of $\X$ is therefore a function defined on $\sphere$ (analogous to $\psi$). By sampling $\X$ at each point in $\data\sites$, we can approximately reconstruct the surface by interpolating each of the components. For more details, see~\cite{Shankar:2015km}.

\subsection{Discretizing force models}

In practice, the RBF-based surface reconstruction is primarily used for discretizing terms in the force models for immersed elastic structures. This requires both evaluating~\eqref{eq:interpolant} at a larger number of points than used to represent the structure, and also approximating derivatives of~\eqref{eq:interpolant} at that larger set of points. We now describe our method for doing so.

Let $\L$ be a generic linear operator. Depending on the context, $\L$ could be an operator that evaluates the interpolant at a larger number of points, or one of the differential operators  $\partial/\partial\q[\mu]$ and $\partial^2/\partial\q[\mu]\partial\q[\lambda]$. In order to approximate $\L \psi$ at the set of sample sites $\sample\sites$, we simply apply $\L$ to the interpolant~\eqref{eq:interpolant} and evaluate t $\sample\sites$ as follows:
\begin{align}
    \left.\L s(\data\Xp)\right|_{\sample\sites}
    := \sum_{i=1}^{\data\cardinality} c_i \left.\L\phi\left(\left\|\data\Xp-\data\Xp_i\right\|\right)\right|_{\sample\sites}
    + \sum_{k=1}^{\poly\cardinality} d_k \left.\L p_k(\data\Xp)\right|_{\sample\sites}.
\end{align}
Define the matrix containing evaluations of $\L\phi$ at $\sample\sites$ to be $L_{\phi}$, and its polynomial counterpart to be $L_p$. Then, the above operation can be written purely in terms of matrix-vector multiplications as
\begin{align}
\left.\L s(\data\Xp)\right|_{\sample\sites} &= L_{\phi} \underline{c} + L_p \underline{d},\\
&= \begin{bmatrix} L_{\phi} & L_p \end{bmatrix} \begin{bmatrix} \underline{c} \\ \underline{d} \end{bmatrix},\\
&= \tilde{L} \tilde{\underline{c}}.
\end{align}
Using the formal definition of $\tilde{\underline{c}} = \tilde{A}^{-1} \tilde{\underline{\psi}}$ from \eqref{eq:rbf_linsys}, we may rewrite this as
\begin{align}
\left.\L s(\data\Xp)\right|_{\sample\sites} &= \tilde{L} \tilde{A}^{-1} \tilde{\underline{\psi}}.
\end{align}
We can now write the product $\tilde{L} \tilde{A}^{-1}$ as a block matrix $\begin{bmatrix} L_{\L} & L_{0} \end{bmatrix}$ so that
\begin{align}
\left.\L s(\data\Xp)\right|_{\sample\sites} &= \begin{bmatrix} L_{\L} & L_0 \end{bmatrix} \begin{bmatrix} \underline{\psi} \\ 0 \end{bmatrix},\\
\implies \left.\L s(\data\Xp)\right|_{\sample\sites} &= L_{\L} \underline{\psi}.
\end{align}
Here, $L_{\L}$ is an $\sample\cardinality \times \data\cardinality$ \emph{operator} matrix whose application to the vector $\underline{\psi}$ approximates application and evaluation of the operator $\L$: $\left.\L \psi(\data\Xp)\right|_{\sample\sites}$. In practice, this matrix is generated by solving systems of the form $\tilde{A} L_{\L} = \tilde{L}^T$ for each operator $\L$; this process can be made more efficient by first computing the $lu$-decomposition of $\tilde{A}$, then solving for the columns of $L_{\L}$. The differentiation-matrix approach has been used for the meshfree solution of PDEs~\cite{Fasshauer:2007ui}, but also in the context of the immersed boundary method~\cite{Shankar:2015km} and the method of regularized Stokeslets~\cite{Olson:2015ja} to sample immersed boundaries or approximate derivatives of positions (for problems in two-dimensional domains). It is important to note that $L_{\L}$ is completely independent of the function $\psi$; in fact, it depends only on the basis functions $\phi$ and $p_k$, the fixed locations $\data\Xp$, and the fixed set of evaluation locations $\sample\Xp$. In this article, our approach is to precompute a separate matrix $L_{\L}$ for each operator $\L$ as a preprocessing step, and then simply apply these matrices to vectors containing samples of any function that needs to be evaluated or differentiated. It is also straightforward to generate versions of $L_{\L}$ that produces derivatives at the data sites $\data\sites$ simply by replacing $\sample\sites$ in the above discussion with $\data\sites$. 

With these operators in hand, the force model is readily discretized. The quantities $\metric_{\alpha\beta}$, $\metric^{\alpha\beta}$, $\dot{\metric}_{\alpha\beta}$, $\n$, $H$, and $K$ require only pointwise first and second derivative data to compute. The matrices $L_{\L}$ are dense, but a parallelized implementation of BLAS can be used to optimize dense matrix vector multiplications involving the $L_{\L}$ matrices. Lagrangian forces can therefore be computed in parallel with few thread synchronizations.

We now have a method for discretizing $\F$ and for computing an appropriate set of points for use in~\eqref{eq:ib-spread}. The following section is devoted to computing integration weights, $\weight[i]$, at each sample site, $\X$, using RBFs.

